[Re] The Discriminative Kalman Filter for Bayesian Filtering with Nonlinear and Non-Gaussian Observation Models

Kalman filters provide a straightforward and interpretable means to estimate hidden or latent variables, and have found numerous applications in control, robotics, signal processing, and machine learning. One such application is neural decoding for neuroprostheses. In 2020, Burkhart et al. thoroughly evaluated their new version of the Kalman filter that leverages Bayes' theorem to improve filter performance for highly non-linear or non-Gaussian observation models. This work provides an open-source Python alternative to the authors' MATLAB algorithm. Specifically, we reproduce their most salient results for neuroscientific contexts and further examine the efficacy of their filter using multiple random seeds and previously unused trials from the authors' dataset. All experiments were performed offline on a single computer.

==> metadata.tex <==
% DO NOT EDIT - automatically generated from metadata.yaml

\def \codeURL{https://github.com/Josuelmet/Discriminative-Kalman-Filter-4.5-Python}
\def \codeDOI{}
\def \codeSWH{}
\def \dataURL{https://portal.nersc.gov/project/crcns/download/dream/data_sets/Flint_2012}
\def \dataDOI{}
\def \editorNAME{}
\def \editorORCID{}
\def \reviewerINAME{}
\def \reviewerIORCID{}
\def \reviewerIINAME{}
\def \reviewerIIORCID{}
\def \dateRECEIVED{}
\def \dateACCEPTED{}
\def \datePUBLISHED{}
\def \articleTITLE{[Re] The Discriminative Kalman Filter for Bayesian Filtering with Nonlinear and Non-Gaussian Observation Models}
\def \articleTYPE{Replication / Computational Neuroscience}
\def \articleDOMAIN{}
\def \articleBIBLIOGRAPHY{bibliography.bib}
\def \articleYEAR{2023}
\def \reviewURL{}
\def \articleABSTRACT{Kalman filters provide a straightforward and interpretable means to estimate hidden or latent variables, and have found numerous applications in control, robotics, signal processing, and machine learning. One such application is neural decoding for neuroprostheses. In 2020, Burkhart et al. thoroughly evaluated their new version of the Kalman filter that leverages Bayes' theorem to improve filter performance for highly non-linear or non-Gaussian observation models. This work provides an open-source Python alternative to the authors' MATLAB algorithm. Specifically, we reproduce their most salient results for neuroscientific contexts and further examine the efficacy of their filter using multiple random seeds and previously unused trials from the authors' dataset. All experiments were performed offline using a single CPU.}
\def \replicationCITE{}
\def \replicationBIB{}
\def \replicationURL{}
\def \replicationDOI{}
\def \contactNAME{Josue Casco-Rodriguez}
\def \contactEMAIL{jc135@rice.edu}
\def \articleKEYWORDS{neuroengineering, neuroscience, kalman, filter, matlab, python, pytorch, regression}
\def \journalNAME{ReScience C}
\def \journalVOLUME{}
\def \journalISSUE{}
\def \articleNUMBER{}
\def \articleDOI{}
\def \authorsFULL{Josue Casco-Rodriguez, Caleb Kemere, Richard G. Baraniuk}
\def \authorsABBRV{J. Casco-Rodriguez, C. Kemere, R. G. Baraniuk}
\def \authorsSHORT{Casco-Rodriguez, Kemere, Baraniuk}
\title{\articleTITLE}
\date{}
\author[1,\orcid{0000-0002-9694-0982}]{Josue Casco-Rodriguez}
\author[1, \orcid{0000-0003-2054-0234}]{Caleb Kemere}
\author[1, \orcid{0000-0002-0721-8999}]{Richard G. Baraniuk}
\affil[1]{Rice University, Houston, Texas, USA}
